Functionalizing Aromatic Compounds with Optical Cycling Centers

Molecular design principles provide guidelines for augmenting a molecule with a smaller group of atoms to realize a desired property or function. We demonstrate that these concepts can be used to create an optical cycling center that can be attached to a number of aromatic ligands, allowing the scattering of many photons from the resulting molecules without changing the molecular vibrational states. We provide further design principles that indicate the ability to expand this work. This represents a significant step towards a quantum functional group, which may serve as a generic qubit moiety that can be attached to a wide range of molecular structures and surfaces.

==> dodiff <==
#!\bin\bash

file=alternatecharging
git show HEAD~6:${file}.tex > lookatold.tex
#git show alex:${file}.tex > lookatold.tex
latexdiff lookatold.tex ${file}.tex > diff.tex
cp ${file}.bib diff.bib
cp ${file}Notes.bib diffNotes.bib
pdflatex diff
bibtex diff||true
pdflatex diff
pdflatex diff
open -a Preview diff.pdf
